Curved Surface Patches for Rough Terrain Perception

Attaining animal-like legged locomotion on rough outdoor terrain with sparse foothold affordances -a primary use-case for legs vs other forms of locomotion- is a largely open problem. New advancements in control and perception have enabled bipeds to walk on flat and uneven indoor environments. But tasks that require reliable contact with unstructured world surfaces, for example walking on natural rocky terrain, need new perception and control algorithms. This thesis introduces 3D perception algorithms for contact tasks such as foot placement in rough terrain environments. We introduce a new method to identify and model potential contact areas between the robot's foot and a surface using a set of bounded curved patches. We present a patch parameterization model and an algorithm to fit and perceptually validate patches to 3D point samples. Having defined the environment representation using the patch model, we introduce a way to assemble patches into a spatial map. This map represents a sparse set of local areas potentially appropriate for contact between the robot and the surface. The process of creating such a map includes sparse seed point sampling, neighborhood searching, as well as patch fitting and validation. Various ways of sampling are introduced including a real time bio-inspired system for finding patches statistically similar to those that humans select while traversing rocky trails. These sparse patch algorithms are integrated with a dense volumetric fusion of range data from a moving depth camera, maintaining a dynamic patch map of relevant contact surfaces around a robot in real time. We integrate and test the algorithms as part of a real-time foothold perception system on a mini-biped robot, performing foot placements on rocks.

==> Acknowledgments.tex <==
%*******************************************************
% Acknowledgments
%*******************************************************
\pdfbookmark[1]{Acknowledgments}{acknowledgments}

\begin{flushright}{\slshape    
    We have seen that computer programming is an art, \\ 
    because it applies accumulated knowledge to the world, \\ 
    because it requires skill and ingenuity, and especially \\
    because it produces objects of beauty.} \\ \medskip
    --- \defcitealias{knuth:1974}{Donald E. Knuth}\citetalias{knuth:1974} \citep{knuth:1974}
\end{flushright}



\bigskip

\begingroup
\let\clearpage\relax
\let\cleardoublepage\relax
\let\cleardoublepage\relax
\chapter*{Acknowledgments}
Put your acknowledgments here.

Many thanks to everybody who already sent me a postcard!

Regarding the typography and other help, many thanks go to Marco 
Kuhlmann, Philipp Lehman, Lothar Schlesier, Jim Young, Lorenzo 
Pantieri and Enrico Gregorio\footnote{Members of GuIT (Gruppo 
Italiano Utilizzatori di \TeX\ e \LaTeX )}, J\"org Sommer, 
Joachim K\"ostler, Daniel Gottschlag, Denis Aydin, Paride 
Legovini, Steffen Prochnow, Nicolas Repp, Hinrich Harms, 
 Roland Winkler, J\"org Weber, 
 and the whole \LaTeX-community for support, ideas and 
 some great software.

\bigskip

\noindent\emph{Regarding \mLyX}: The \mLyX\ port was intially done by 
\emph{Nicholas Mariette} in March 2009 and continued by 
\emph{Ivo Pletikosi\'c} in 2011. Thank you very much for your 
work and the contributions to the original style.


\endgroup





==> Acronyms.tex <==
\chapter*{List of Symbols and Notations}
\begin{acronym}[UML]
  \acro{$m_x$}{TBD}
\end{acronym} 

==> Colophon.tex <==
\pagestyle{empty}
\hfill
\vfill

\pdfbookmark[0]{Colophon}{colophon}
\section*{Colophon}
This document was typeset using the \texttt{classicthesis} \footnote{\url{http://code.google.com/p/classicthesis/}} template in \LaTeX\ developed by Andr\'e Miede and inspired by Robert Bringhurst's seminal book on typography ``\emph{The Elements of Typographic Style}''.

==> Declaration.tex <==
%*******************************************************
% Declaration
%*******************************************************
\refstepcounter{dummy}
\pdfbookmark[0]{Declaration}{declaration}
\chapter*{Declaration}
\thispagestyle{empty}
Put your declaration here.
\bigskip
 
\noindent\textit{\myLocation, \myTime}

\smallskip

\begin{flushright}
    \begin{tabular}{m{5cm}}
        \\ \hline
        \centering\myName \\
    \end{tabular}
\end{flushright}


==> DirtyTitlepage.tex <==
%*******************************************************
% Little Dirty Titlepage
%*******************************************************
\thispagestyle{empty}
%\pdfbookmark[1]{Titel}{title}
%*******************************************************
\begin{center}
    \spacedlowsmallcaps{\myName} \\ \medskip                        

    \begingroup
        \color{Maroon}\spacedallcaps{\myTitle}
    \endgroup
\end{center}        


==> related.tex <==
\section{Related Work}

\subsection{Legged Robot Locomotion on Rough Terrain}
In a sequence of papers \cite{Belter09, BLS10, WB11, BS11} Belter et al. study hexapod robot locomotion on rough terrain.  In particular, in \cite{Belter09} an adaptive foothold selection algorithm is introduced for avoiding slippages.  Given the model of the environment as 3D point cloud input, both a global dense grid elevation map and a decision surface are constructed.  The decision surface is a polynomial that is constructed taking into account different types of coefficients that represent properties of the terrain, e.g. slope or distance from the center of the map.  The process includes an unsupervised learning process where the robot learns offline the correspondence between the coefficients and the slippage of the environment.  The adaptive foothold selection uses a local elevation map around the robot and the decision surface.  A simple tripod control algorithm is used for the locomotion, which makes the robot statically stable.  The algorithm is applied both in simulation and on real hexapod robots (Ragno and Messor).  In \cite{BLS10}, the authors added the perception part using a structured light sensor, providing also methods for recovering missing data using filtering on the elevation map.  In \cite{BS11}, a 2D laser scanner is used for data acquisition for the local moving grid and filters for spatially isolated and mixed pixels is applied, w the elevation map is updated when the robot is moving.  The results prove that holes and flat areas are appropriate for footholds, so that you can avoid slippages, which is not surprising. In \cite{WB11}, TBD

Problems: 1) Even the map is built in real-time, reasoning the contact between six legs and the environment is required.  Footholds close to nominal placements (using e.g. the tripod gait control) are selected . The algorithm does not consider the uncertainty of the data, although it filters out fraud points.

\subsection{Salient Point}
TBD

\subsection{Local Properties of the Environment}
TBD

\subsection{Filtering the Input Data}
TBD
